Quasi-optimal hierarchically semi-separable matrix approximation

We present a randomized algorithm for producing a quasi-optimal hierarchically semi-separable (HSS) approximation to an $N\times N$ matrix $A$ using only matrix-vector products with $A$ and $A^T$. We prove that, using $O(k \log(N/k))$ matrix-vector products and ${O}(N k^2 \log(N/k))$ additional runtime, the algorithm returns an HSS matrix $B$ with rank-$k$ blocks whose expected Frobenius norm error $\mathbb{E}[\|A - B\|_F^2]$ is at most $O(\log(N/k))$ times worse than the best possible approximation error by an HSS rank-$k$ matrix. In fact, the algorithm we analyze in a simple modification of an empirically effective method proposed by [Levitt & Martinsson, SISC 2024]. As a stepping stone towards our main result, we prove two results that are of independent interest: a similar guarantee for a variant of the algorithm which accesses $A$'s entries directly, and explicit error bounds for near-optimal subspace approximation using projection-cost-preserving sketches. To the best of our knowledge, our analysis constitutes the first polynomial-time quasi-optimality result for HSS matrix approximation, both in the explicit access model and the matrix-vector product query model.

==> bib_macros.tex <==
  % branched from Michael Forbes' macro document
  % September 2014
  \usepackage{nth}
  \usepackage{intcalc}

  \newcommand{\cSTOC}[1]{\nth{\intcalcSub{#1}{1968}}\ Annual\ ACM\ Symposium\ on\ Theory\ of\ Computing\ (STOC)}
  \newcommand{\cFSTTCS}[1]{\nth{\intcalcSub{#1}{1980}}\ International\ Conference\ on\ Foundations\ of\ Software\ Technology\ and\ Theoretical\ Computer\ Science\ (FSTTCS)}
  \newcommand{\cCCC}[1]{\nth{\intcalcSub{#1}{1985}}\ Annual\ IEEE\ Conference\ on\ Computational\ Complexity\ (CCC)}
  \newcommand{\cFOCS}[1]{\nth{\intcalcSub{#1}{1959}}\ Annual\ IEEE\ Symposium\ on\ Foundations\ of\ Computer\ Science\ (FOCS)}
  \newcommand{\cRANDOM}[1]{\nth{\intcalcSub{#1}{1996}}\ International\ Workshop\ on\ Randomization\ and\ Computation\ (RANDOM)}
  \newcommand{\cISSAC}[1]{#1\ International\ Symposium\ on\ Symbolic\ and\ Algebraic\ Computation\ (ISSAC)}
  \newcommand{\cICALP}[1]{\nth{\intcalcSub{#1}{1973}}\ International\ Colloquium\ on\ Automata,\ Languages and\ Programming\ (ICALP)}
  \newcommand{\cCOLT}[1]{\nth{\intcalcSub{#1}{1987}}\ Annual\ Conference\ on\ Computational\ Learning\ Theory\ (COLT)}
  \newcommand{\cCSR}[1]{\nth{\intcalcSub{#1}{2005}}\ International\ Computer\ Science\ Symposium\ in\ Russia\ (CSR)}
  \newcommand{\cMFCS}[1]{\nth{\intcalcSub{#1}{1975}}\ International\ Symposium\ on\ the\ Mathematical\ Foundations\ of\ Computer\ Science\ (MFCS)}
  \newcommand{\cPODS}[1]{\nth{\intcalcSub{#1}{1981}}\ Symposium\ on\ Principles\ of\ Database\ Systems\ (PODS)}
  \newcommand{\cSODA}[1]{\nth{\intcalcSub{#1}{1989}}\ Annual\ ACM-SIAM\ Symposium\ on\ Discrete\ Algorithms\ (SODA)}
  \newcommand{\cNIPS}[1]{Advances\ in\ Neural\ Information\ Processing\ Systems\ \intcalcSub{#1}{1987} (NeurIPS)}
  \newcommand{\cWALCOM}[1]{\nth{\intcalcSub{#1}{2006}}\ International\ Workshop\ on\ Algorithms\ and\ Computation\ (WALCOM)}
  \newcommand{\cSoCG}[1]{\nth{\intcalcSub{#1}{1984}}\ Annual\ Symposium\ on\ Computational\ Geometry\ (SCG)}
  \newcommand{\cKDD}[1]{\nth{\intcalcSub{#1}{1994}}\ ACM\ SIGKDD\ International\ Conference\ on\ Knowledge\ Discovery\ and\ Data\ Mining\ (KDD)}
  \newcommand{\cICML}[1]{\nth{\intcalcSub{#1}{1983}}\ International\ Conference\ on\ Machine\ Learning\ (ICML)}
  \newcommand{\cAISTATS}[1]{\nth{\intcalcSub{#1}{1997}}\ International\ Conference\ on\ Artificial\ Intelligence\ and\ Statistics\ (AISTATS)}
  \newcommand{\cITCS}[1]{\nth{\intcalcSub{#1}{2009}}\ Conference\ on\ Innovations\ in\ Theoretical\ Computer\ Science\ (ITCS)}
  \newcommand{\cPODC}[1]{{#1}\ ACM\ Symposium\ on\ Principles\ of\ Distributed\ Computing\ (PODC)}
  \newcommand{\cAPPROX}[1]{\nth{\intcalcSub{#1}{1997}}\ International\ Workshop\ on\ Approximation\ Algorithms\ for\  Combinatorial\ Optimization\ Problems\ (APPROX)}
  \newcommand{\cSTACS}[1]{\nth{\intcalcSub{#1}{1983}}\ International\ Symposium\ on\ Theoretical\ Aspects\ of\  Computer\ Science\ (STACS)}
  \newcommand{\cMTNS}[1]{\nth{\intcalcSub{#1}{1991}}\ International\ Symposium\ on\ Mathematical\ Theory\ of\  Networks\ and\ Systems\ (MTNS)}
  \newcommand{\cICM}[1]{International\ Congress\ of\ Mathematicians\ {#1} (ICM)}
  \newcommand{\cWWW}[1]{\nth{\intcalcSub{#1}{1991}}\ International\ World\ Wide\ Web\ Conference\ (WWW)}
  \newcommand{\cICLR}[1]{\nth{\intcalcSub{#1}{2012}}\ International\ Conference\ on\ Learning\ Representations\ (ICLR)}
  \newcommand{\cICCV}[1]{\nth{\intcalcSub{#1}{1994}}\ IEEE\ International\ Conference\ on\ Computer\ Vision\ (ICCV)}
  \newcommand{\cICASSP}[1]{#1\ International\ Conference\ on\ Acoustics,\ Speech,\ and\ Signal\ Processing\ (ICASSP)}
  \newcommand{\cUAI}[1]{\nth{\intcalcSub{#1}{1984}}\ Annual\ Conference\ on\ Uncertainty\ in\ Artificial\ Intelligence\ (UAI)}
  \newcommand{\cSOSA}[1]{\nth{\intcalcSub{#1}{2017}}\ Symposium\ on\ Simplicity\ in\ Algorithms\ (SOSA)}
  \newcommand{\cISIT}[1]{#1\ IEEE\ International\ Symposium\ on\ Information\ Theory\ (ISIT)}  
  \newcommand{\cALT}[1]{\nth{\intcalcSub{#1}{1989}}\ International\ Conference\ on\ Algorithmic\ Learning\ Theory\ (ALT)} 
  \newcommand{\cWSDM}[1]{\nth{\intcalcSub{#1}{2007}}\ International\ Conference\ on\ Web\ Search\ and\ Data\ Mining\ (WSDM)} 
  \newcommand{\cICDM}[1]{#1\ IEEE\ International\ Conference\ on\ Data\ Mining\ (ICDM)}  
  \newcommand{\cEC}[1]{\nth{\intcalcSub{#1}{1999}}\ ACM\ Conference\ on\ Economics\ and\ Computation\ (EC)} 
  \newcommand{\cDISC}[1]{\nth{\intcalcSub{#1}{1986}}\ International\ Symposium\ on\ Distributed\ Computing\ (DISC)}
  \newcommand{\cSIGMOD}[1]{{#1} ACM SIGMOD International Conference on Management of Data}
  \newcommand{\cCIKM}[1]{\nth{\intcalcSub{#1}{1991}}\ ACM\ International\ Conference\ on\ Information\ and\ Knowledge\ Management\ (CIKM)}
  \newcommand{\cAAAI}[1]{AAAI\ Conference\ on\ Artificial (AAAI)}  
  \newcommand{\cICDE}[1]{\nth{\intcalcSub{#1}{1984}}\ IEEE\ International\ Conference\ on\ Data\ Engineering\ (ICDE)}  
  \newcommand{\cSPAA}[1]{\nth{\intcalcSub{#1}{1988}}\ ACM\ Symposium\ on\ Parallel\ Algorithms\ and\ Architectures\ (SPAA)}  
  \newcommand{\cESA}[1]{\nth{\intcalcSub{#1}{1992}}\ European\ Symposium\ on\ Algorithms\ (ESA)}  

  \newcommand{\pSTOC}[1]{Preliminary\ version\ in\ the\ \cSTOC{#1}}
  \newcommand{\pFSTTCS}[1]{Preliminary\ version\ in\ the\ \cFSTTCS{#1}}
  \newcommand{\pCCC}[1]{Preliminary\ version\ in\ the\ \cCCC{#1}}
  \newcommand{\pFOCS}[1]{Preliminary\ version\ in\ the\ \cFOCS{#1}}
  \newcommand{\pRANDOM}[1]{Preliminary\ version\ in\ the\ \cRANDOM{#1}}
  \newcommand{\pISSAC}[1]{Preliminary\ version\ in\ the\ \cISSAC{#1}}
  \newcommand{\pICALP}[1]{Preliminary\ version\ in\ the\ \cICALP{#1}}
  \newcommand{\pCOLT}[1]{Preliminary\ version\ in\ the\ \cCOLT{#1}}
  \newcommand{\pCSR}[1]{Preliminary\ version\ in\ the\ \cCSR{#1}}
  \newcommand{\pMFCS}[1]{Preliminary\ version\ in\ the\ \cMFCS{#1}}
  \newcommand{\pPODS}[1]{Preliminary\ version\ in\ the\ \cPODS{#1}}
  \newcommand{\pSODA}[1]{Preliminary\ version\ in\ the\ \cSODA{#1}}
  \newcommand{\pNIPS}[1]{Preliminary\ version\ in\ \cNIPS{#1}}
  \newcommand{\pWALCOM}[1]{Preliminary\ version\ in\ the\ \cWALCOM{#1}}
  \newcommand{\pSoCG}[1]{Preliminary\ version\ in\ the\ \cSoCG{#1}}
  \newcommand{\pKDD}[1]{Preliminary\ version\ in\ the\ \cKDD{#1}}
  \newcommand{\pICML}[1]{Preliminary\ version\ in\ the\ \cICML{#1}}
  \newcommand{\pAISTATS}[1]{Preliminary\ version\ in\ the\ \cAISTATS{#1}}
  \newcommand{\pITCS}[1]{Preliminary\ version\ in\ the\ \cITCS{#1}}
  \newcommand{\pPODC}[1]{Preliminary\ version\ in\ the\ \cPODC{#1}}
  \newcommand{\pAPPROX}[1]{Preliminary\ version\ in\ the\ \cAPPROX{#1}}
  \newcommand{\pSTACS}[1]{Preliminary\ version\ in\ the\ \cSTACS{#1}}
  \newcommand{\pMTNS}[1]{Preliminary\ version\ in\ the\ \cMTNS{#1}}
  \newcommand{\pICM}[1]{Preliminary\ version\ in\ the\ \cICM{#1}}
  \newcommand{\pWWW}[1]{Preliminary\ version\ in\ the\ \cWWW{#1}}
  \newcommand{\pICLR}[1]{Preliminary\ version\ in\ the\ \cICLR{#1}}
  \newcommand{\pICCV}[1]{Preliminary\ version\ in\ the\ \cICCV{#1}}
  \newcommand{\pICASSP}[1]{Preliminary\ version\ in\ the\ \cICASSP{#1}}
  \newcommand{\pUAI}[1]{Preliminary\ version\ in\ the\ \cUAI{#1}, #1}
  \newcommand{\pSOSA}[1]{Preliminary\ version\ in\ the\ \cSOSA{#1}, #1}
  \newcommand{\pISIT}[1]{Preliminary\ version\ in\ the\ \cISIT{#1}}
  \newcommand{\pALT}[1]{Preliminary\ version\ in\ the\ \cALT{#1}}
  \newcommand{\pWSDM}[1]{Preliminary\ version\ in\ the\ \cWSDM{#1}}
  \newcommand{\pICDM}[1]{Preliminary\ version\ in\ the\ \cICDM{#1}}
  \newcommand{\pEC}[1]{Preliminary\ version\ in\ the\ \cEC{#1}}
  \newcommand{\pDISC}[1]{Preliminary\ version\ in\ the\ \cDISC{#1}, #1}
  \newcommand{\pSIGMOD}[1]{Preliminary\ version\ in\ the\ \cSIGMOD{#1}, #1}
  \newcommand{\pCIKM}[1]{Preliminary\ version\ in\ the\ \cCIKM{#1}, #1}
  \newcommand{\pAAAI}[1]{Preliminary\ version\ in\ the\ \cAAAI{#1}, #1}
  \newcommand{\pICDE}[1]{Preliminary\ version\ in\ the\ \cICDE{#1}, #1}
  \newcommand{\pSPAA}[1]{Preliminary\ version\ in\ the\ \cSPAA{#1}, #1}
    \newcommand{\pESA}[1]{Preliminary\ version\ in\ the\ \cESA{#1}, #1}



  \newcommand{\STOC}[1]{Proceedings\ of\ the\ \cSTOC{#1}}
  \newcommand{\FSTTCS}[1]{Proceedings\ of\ the\ \cFSTTCS{#1}}
  \newcommand{\CCC}[1]{Proceedings\ of\ the\ \cCCC{#1}}
  \newcommand{\FOCS}[1]{Proceedings\ of\ the\ \cFOCS{#1}}
  \newcommand{\RANDOM}[1]{Proceedings\ of\ the\ \cRANDOM{#1}}
  \newcommand{\ISSAC}[1]{Proceedings\ of\ the\ \cISSAC{#1}}
  \newcommand{\ICALP}[1]{Proceedings\ of\ the\ \cICALP{#1}}
  \newcommand{\COLT}[1]{Proceedings\ of\ the\ \cCOLT{#1}}
  \newcommand{\CSR}[1]{Proceedings\ of\ the\ \cCSR{#1}}
  \newcommand{\MFCS}[1]{Proceedings\ of\ the\ \cMFCS{#1}}
  \newcommand{\PODS}[1]{Proceedings\ of\ the\ \cPODS{#1}}
  \newcommand{\SODA}[1]{Proceedings\ of\ the\ \cSODA{#1}}
  \newcommand{\NIPS}[1]{\cNIPS{#1}}
  \newcommand{\WALCOM}[1]{Proceedings\ of\ the\ \cWALCOM{#1}}
  \newcommand{\SoCG}[1]{Proceedings\ of\ the\ \cSoCG{#1}}
  \newcommand{\KDD}[1]{Proceedings\ of\ the\ \cKDD{#1}}
  \newcommand{\ICML}[1]{Proceedings\ of\ the\ \cICML{#1}}
  \newcommand{\AISTATS}[1]{Proceedings\ of\ the\ \cAISTATS{#1}}
  \newcommand{\ITCS}[1]{Proceedings\ of\ the\ \cITCS{#1}}
  \newcommand{\PODC}[1]{Proceedings\ of\ the\ \cPODC{#1}}
  \newcommand{\APPROX}[1]{Proceedings\ of\ the\ \cAPPROX{#1}}
  \newcommand{\STACS}[1]{Proceedings\ of\ the\ \cSTACS{#1}}
  \newcommand{\MTNS}[1]{Proceedings\ of\ the\ \cMTNS{#1}}
  \newcommand{\ICM}[1]{Proceedings\ of\ the\ \cICM{#1}}
  \newcommand{\WWW}[1]{Proceedings\ of\ the\ \cWWW{#1}}
  \newcommand{\ICLR}[1]{Proceedings\ of\ the\ \cICLR{#1}}
  \newcommand{\ICCV}[1]{Proceedings\ of\ the\ \cICCV{#1}}
  \newcommand{\ICASSP}[1]{Proceedings\ of\ the\ \cICASSP{#1}}
  \newcommand{\UAI}[1]{Proceedings\ of\ the\ \cUAI{#1}}
  \newcommand{\SOSA}[1]{Proceedings\ of\ the\ \cSOSA{#1}}
  \newcommand{\ISIT}[1]{Proceedings\ of\ the\ \cISIT{#1}}
  \newcommand{\ALT}[1]{Proceedings\ of\ the\ \cALT{#1}}
  \newcommand{\WSDM}[1]{Proceedings\ of\ the\ \cWSDM{#1}}
  \newcommand{\ICDM}[1]{Proceedings\ of\ the\ \cICDM{#1}}
  \newcommand{\EC}[1]{Proceedings\ of\ the\ \cEC{#1}}
  \newcommand{\DISC}[1]{Proceedings\ of\ the\ \cDISC{#1}}
  \newcommand{\SIGMOD}[1]{Proceedings\ of\ the\ \cSIGMOD{#1}}
  \newcommand{\CIKM}[1]{Proceedings\ of\ the\ \cCIKM{#1}}
  \newcommand{\AAAI}[1]{Proceedings\ of\ the\ \cAAAI{#1}}
  \newcommand{\ICDE}[1]{Proceedings\ of\ the\ \cICDE{#1}}
  \newcommand{\SPAA}[1]{Proceedings\ of\ the\ \cSPAA{#1}}
  \newcommand{\ESA}[1]{Proceedings\ of\ the\ \cESA{#1}}


  \newcommand{\arXiv}[1]{\href{http://arxiv.org/abs/#1}{arXiv:#1}}
  \newcommand{\farXiv}[1]{Full\ version\ at\ \arXiv{#1}}
  \newcommand{\parXiv}[1]{Preliminary\ version\ at\ \arXiv{#1}}
  \newcommand{\CoRR}{Computing\ Research\ Repository\ (CoRR)}

  \newcommand{\cECCC}[2]{\href{http://eccc.hpi-web.de/report/20#1/#2/}{Electronic\ Colloquium\ on\ Computational\ Complexity\ (ECCC),\ Technical\ Report\ TR#1-#2}}
  \newcommand{\ECCC}{Electronic\ Colloquium\ on\ Computational\ Complexity\ (ECCC)}
  \newcommand{\fECCC}[2]{Full\ version\ in\ the\ \cECCC{#1}{#2}}
  \newcommand{\pECCC}[2]{Preliminary\ version\ in\ the\ \cECCC{#1}{#2}}

==> imgs/HBS_def.tex <==

\begin{tikzpicture}
   
    \draw[fill=black!20] (0,0) rectangle (8,8);

    \draw[fill=black!10] (0,0) rectangle (4,4);
    \draw[fill=black!10] (4,4) rectangle (8,8);

    \draw[fill=black!10] (0,4) rectangle (2,6);
    \draw[fill=black!10] (2,6) rectangle (4,8);
    \draw[fill=black!10] (4,0) rectangle (6,2);
    \draw[fill=black!10] (6,2) rectangle (8,4);
   
    \draw[fill=black!10] (0,6) rectangle (1,7);
    \draw[fill=black!10] (1,7) rectangle (2,8);
    \draw[fill=black!10] (2,4) rectangle (3,5);
    \draw[fill=black!10] (3,5) rectangle (4,6);
    \draw[fill=black!10] (4,2) rectangle (5,3);
    \draw[fill=black!10] (5,3) rectangle (6,4);
    \draw[fill=black!10] (6,0) rectangle (7,1);
    \draw[fill=black!10] (7,1) rectangle (8,2);


    \draw[color=c1,line width=2pt,pattern=north west lines, pattern color = c1!40] (0,6) rectangle (1,7);
    \draw[color=c1,line width=2pt,pattern=north west lines, pattern color = c1!40] (2,6) rectangle (8,7);
    % \draw[color=c1,line width=2pt,pattern=north west lines, pattern color = c1!40] (2,6) rectangle (4,7);
    % \draw[color=c1,line width=2pt,pattern=north west lines, pattern color = c1!40] (4,6) rectangle (8,7);


    \draw[color=c0,line width=2pt,pattern=north east lines, pattern color = c0!40] (5,0) rectangle (6,2);
    \draw[color=c0,line width=2pt,pattern=north east lines, pattern color = c0!40] (5,3) rectangle (6,8);
    % \draw[color=c0,line width=2pt,pattern=north east lines, pattern color = c0!40] (5,3) rectangle (6,4);
    % \draw[color=c0,line width=2pt,pattern=north east lines, pattern color = c0!40] (5,4) rectangle (6,8);
\end{tikzpicture}

==> imgs/HODLR_def.tex <==
\begin{tikzpicture}
   
    \draw[fill=black!20] (0,0) rectangle (8,8);

    \draw[fill=black!10] (0,0) rectangle (4,4);
    \draw[fill=black!10] (4,4) rectangle (8,8);

    \draw[fill=black!10] (0,4) rectangle (2,6);
    \draw[fill=black!10] (2,6) rectangle (4,8);
    \draw[fill=black!10] (4,0) rectangle (6,2);
    \draw[fill=black!10] (6,2) rectangle (8,4);
   
    \draw[fill=black!10] (0,6) rectangle (1,7);
    \draw[fill=black!10] (1,7) rectangle (2,8);
    \draw[fill=black!10] (2,4) rectangle (3,5);
    \draw[fill=black!10] (3,5) rectangle (4,6);
    \draw[fill=black!10] (4,2) rectangle (5,3);
    \draw[fill=black!10] (5,3) rectangle (6,4);
    \draw[fill=black!10] (6,0) rectangle (7,1);
    \draw[fill=black!10] (7,1) rectangle (8,2);

\end{tikzpicture}


==> imgs/HSS_def_old.tex <==
\begin{tikzpicture}
   
    \draw[fill=black!20] (0,0) rectangle (8,8);

\end{tikzpicture}
\hspace{3em}
\begin{tikzpicture}
   
    \draw[fill=black!20] (0,0) rectangle (8,8);

    \draw[fill=black!10] (0,0) rectangle (4,4);
    \draw[fill=black!10] (4,4) rectangle (8,8);

\end{tikzpicture}
\hspace{3em}
\begin{tikzpicture}
   
    \draw[fill=black!20] (0,0) rectangle (8,8);

    \draw[fill=black!10] (0,0) rectangle (4,4);
    \draw[fill=black!10] (4,4) rectangle (8,8);

    \draw[fill=black!10] (0,4) rectangle (2,6);
    \draw[fill=black!10] (2,6) rectangle (4,8);
    \draw[fill=black!10] (4,0) rectangle (6,2);
    \draw[fill=black!10] (6,2) rectangle (8,4);
   
\end{tikzpicture}
\hspace{3em}
\begin{tikzpicture}
   
    \draw[fill=black!20] (0,0) rectangle (8,8);

    \draw[fill=black!10] (0,0) rectangle (4,4);
    \draw[fill=black!10] (4,4) rectangle (8,8);

    \draw[fill=black!10] (0,4) rectangle (2,6);
    \draw[fill=black!10] (2,6) rectangle (4,8);
    \draw[fill=black!10] (4,0) rectangle (6,2);
    \draw[fill=black!10] (6,2) rectangle (8,4);
   
    \draw[fill=black!10] (0,6) rectangle (1,7);
    \draw[fill=black!10] (1,7) rectangle (2,8);
    \draw[fill=black!10] (2,4) rectangle (3,5);
    \draw[fill=black!10] (3,5) rectangle (4,6);
    \draw[fill=black!10] (4,2) rectangle (5,3);
    \draw[fill=black!10] (5,3) rectangle (6,4);
    \draw[fill=black!10] (6,0) rectangle (7,1);
    \draw[fill=black!10] (7,1) rectangle (8,2);

\end{tikzpicture}
